Handling Constrained Optimization in Factor Graphs for Autonomous Navigation

Factor graphs are graphical models used to represent a wide variety of problems across robotics, such as Structure from Motion (SfM), Simultaneous Localization and Mapping (SLAM) and calibration. Typically, at their core, they have an optimization problem whose terms only depend on a small subset of variables. Factor graph solvers exploit the locality of problems to drastically reduce the computational time of the Iterative Least-Squares (ILS) methodology. Although extremely powerful, their application is usually limited to unconstrained problems. In this paper, we model constraints over variables within factor graphs by introducing a factor graph version of the method of Lagrange Multipliers. We show the potential of our method by presenting a full navigation stack based on factor graphs. Differently from standard navigation stacks, we can model both optimal control for local planning and localization with factor graphs, and solve the two problems using the standard ILS methodology. We validate our approach in real-world autonomous navigation scenarios, comparing it with the de facto standard navigation stack implemented in ROS. Comparative experiments show that for the application at hand our system outperforms the standard nonlinear programming solver Interior-Point Optimizer (IPOPT) in runtime, while achieving similar solutions.

==> 2022_paper_bazzana_ral_intro.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{abstract}
\gls{ils} is a common approach to factor graph optimization. In this paper, we model constraints over variables within factor graphs, thus extending factor graph optimization to capture an enlarged class of problems. We show the power of our method by presenting a full navigation stack based on factor graphs.  A navigation stack comprises both motion planning and localization modules that typically use heterogeneous algorithms.  Here instead \gls{mpc} and localization are modeled using the same formalism and solved by using an unmodified
  version of our \gls{ils} solver.
  Experimental results on a real robot show the feasibility of our work,
  and statistically significant comparative experiments against the de facto standard ROS
  \verb+amcl+ - \verb+move_base+  are promising. 
\end{abstract}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Introduction}
\label{sec:intro}
Factor graphs are general graphical formalism to model several
problems.  The robotics community extensively used factor graphs to
approach estimation problems, such as \gls{sfm}, \gls{slam}
and calibration.  Well-known
methodologies to solve large factor graphs use variants of Iterative Least
Squares (\gls{ils})~\cite{kuemmerle2011icra, kaess2008tro, grisetti2020solver} that does not support \emph{constrained} optimization in its original formulation.
Leveraging on the results of~\cite{sodhi2020icra}, in this paper we
present an iterative version of the Lagrange Multipliers method where constraints are modeled as a new class of factors.
Being able to perform constrained optimization allows to extend the
domain of factor graphs to optimal control problems and, hence, to \gls{mpc} \cite{Alessio2009}.  As a result, localization and motion planning can be addressed within a single framework as in the navigation stack we are presenting in this paper, where we use the same solver for both problems. 

Our
system models the localization problem as scan matching with implicit
data association where the likelihood of the current estimate is evaluated through the distance between the scan and the map.  Experimental results show that, given the odometry as initial guess, this method is more
accurate than the Adaptive Monte Carlo Localization ROS package \verb+amcl+\footnote{\url{http://wiki.ros.org/amcl}}, at a
comparable runtime.
\begin{figure}[ht]
	%  \begin{tabular}{cc}
		\centering
		\includegraphics[width=0.15\textwidth]{./pics/obs_with_graph.pdf}
		\hspace{15px}
		\includegraphics[width=0.2\textwidth]{./pics/orazio_cropped.png}
		%  \end{tabular}
	\caption{Left: a trajectory executed by our real robot avoiding an unforeseen obstacle, a schematic factor graph is superposed to it where some robot states are represented (pink circles). Both the localization problem (orange square) and the optimal control are depicted. States are linked by the motion model (yellow squares) and subject to obstacle avoidance and trajectory tracking (green squares). Right: our custom made unicycle.}
	\label{fig:motivation}
	\vspace{-10px}
\end{figure}
Furthermore, to illustrate the effect of our constraint factors we
address the problem of generating a collision free trajectory for a differential drive robot with actuation limits in a dynamic
environment.  
We formulate this problem as an optimal control problem, that is
represented by means of a factor graph comprising the novel \emph{constraint} factors and our proposal of obstacle avoidance factors based on minimization of an artificial potential function~\cite{sfeir2011rose}\cite{farid2017ivs}.

%\begin{figure}[ht]
%	\begin{tabularx}	{0.5\textwidth} { m{3cm} X X }
%	%  \begin{tabular}{cc}
%		\includegraphics[width=0.15\textwidth, valign=c]{./pics/real_robot_experiments/obs_20220228_1103/obs_with_graph.pdf}
%		&
%		\vspace{-22px}
%		\hspace{2px}
%		\includegraphics[width=0.2\textwidth, valign = c]{./pics/orazio_cropped.png}
%		%  \end{tabular}
%\end{tabularx}
%\end{figure}





We validated our approach by running our system on a custom made
robot, where all software runs on a Raspberry PI
4. On the one hand
these real-world experiments show the feasibility of our approach, on
the other hand they highlight its moderate computational requirements.
\figref{fig:motivation} shows a real-world trajectory and a simplistic representation of the related factor graph.
We compare our systems with the well-known ROS navigation stack,
combining \verb+amcl+ for localization and \verb+move_base+\footnote{\url{http://wiki.ros.org/move_base}} for motion planning with the \verb+teb_local_planner+\footnote{\url{http://wiki.ros.org/teb_local_planner}}, the Timed Elastic Band~\cite{rosmann2013ecmr} ROS plugin.  

We performed statistical simulated experiments lasting more than $12$
hours of travel, by cyclically reaching a set of goals in the map of our department. To simulate both structural changes and dynamic environment, we place a set of unmodeled
obstacles.  These experiments show that, despite its simplicity, our
factor graph-based localization is more accurate than
\verb+amcl+, when no global localization is required.
Our \gls{mpc} implementation is always able to reach the goals while
satisfying the control constraints.  Comparative experiments with respect to the aforementioned \verb+move_base+ setup are promising.

In summary, this paper proposes a novel formulation for approaching and
modeling constrained optimization problems with factor graphs.  We
demonstrate our method by implementing core components of a full
navigation stack and we run comparative experiments against highly
engineered systems.

The rest of the paper is organized as follows. \secref{sec:related} discusses the literature on motion planning using factor graphs,
\secref{sec:problem-definition} recaps factor graph optimization particularly focusing on \gls{ils}. \secref{sec:localization} and \secref{sec:mpc} introduce our approach to localization and \gls{mpc} respectively. \secref{sec:approach-constraint} exposes how we model constraints using factor graphs and concludes the theoretical part, \secref{sec:experiments} contains the experiments and results, and \secref{sec:conclusions} concludes the paper.


==> 2022_paper_bazzana_ral_related.tex <==
\newcommand{reviewed}[1]{\textcolor{#1}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Related Work}\label{sec:related}



Factor graphs are a very powerful tool to model a great variety of
optimization problems, spacing from \gls{slam} to \gls{sfm}. In
the recent literature, they have been applied to model optimal control
problems as well \cite{yang2020arxiv, ta2014icuas, xie2020, mukadam2019steap, dong2016planning}.
Formalizing optimal control problems using factor graphs allows to
unify the dual problems of estimation and control under the same
representation.  Thanks to this unification, these two aspects can be addressed jointly taking advantage of efficient \gls{fgs}~\cite{kaess2008tro, kuemmerle2011icra, grisetti2020solver}.

In \cite{mukadam2019steap}, Mukadam et al.~\emph{et al.} managed to
optimize a unique factor graph for both trajectory estimation and
motion planning, where trajectories were modeled using continuous
Gaussian Processes \cite{dong2018sparsegp}. Differently from
\cite{mukadam2019steap}, our approach computes the control inputs, thus
eliminating the need of a controller to track the optimized
trajectory, and supports nonholonomic and inequality constraints.

Mukadam et al.~\emph{et al.} optimize a unique factor graph for both trajectory estimation and
motion planning, where trajectories \reviewed{are} modeled using continuous
Gaussian Processes \cite{dong2018sparsegp}. \reviewed{However, obstacle avoidance is handled through additional terms in the cost function, without being explicitly modeled as a hard constraint. Moreover, the output trajectory does not take into account kinematic constraints, which must be handled by an ad-hoc controller. Conversely, our approach computes the control inputs directly and explicitly model nonholonomic and inequality constraints.}

Including control inputs in a factor graph imposes to address
actuation constraints, that are not handled by common \gls{fgs}. To this
extent a recent work of Yang~\emph{et al.}~\cite{yang2020arxiv}
aims at solving the Linear Quadratic Regulator problems subject to
auxiliary equality constraints using factor graphs. In particular this
work shows how to perform variable elimination to ensure constraint
satisfaction. A solver for constrained optimization is required during
the variable elimination process: the authors suggest to use a
modified version of Gram-Schmidt algorithm.  Our work adds to
\cite{yang2020arxiv} an extension of \gls{ils} for constrained optimization,
where both equality and inequality constrains are tackled.

Xie \emph{et al.}~\cite{xie2020}  further investigate factor graphs to
represent optimal control problems. They introduce Dynamic Factor
Graphs (DFGs) to represent the structure of the dynamic constraints.
To convert the constrained problem into an unconstrained one, they
use the log residual error for equality constraints and the log of a
hinge loss approximation of the residual error for the inequality
constraints.  In contrast, our work leverages on the well-known
method of the Lagrange multipliers for constrained optimization, and
introduces a novel compact and effective way of modeling obstacle
avoidance factors.



\gls{mpc} is one of the most dominant paradigms in automatic control.  An
\gls{mpc} controller aims at predicting the most likely evolution of the states and the
controls that minimize a given cost function over the predefined time
horizon.  It solves a new optimization problem each time by
incorporating the most recent measurements.  Nowadays the application of \gls{mpc}
ranges from automotive to process automation, as well as smart
electricity grids and robotics.  To the best of our knowledge,
Ta~\emph{et al.}~\cite{ta2014icuas} have been the first to address
\gls{mpc} with factor graphs.  They approach optimal control problems
subject to nonlinear equality constraints by introducing a factor
graph formulation of Sequential Quadratic Programming.  Our work
extends \cite{ta2014icuas} by modeling inequality constraints.

Sodhi~\emph{et. al}~\cite{sodhi2020icra} proposes an approach to refine the estimate of past trajectories: to accomplish collision-free trajectories, states are subject to inequality constraints.  To the best of our knowledge they have been the first to 
introduce the use of Lagrange Multipliers in the context of
incremental smoothing.  We rely on the same concepts, and we extend
the approach to represent general equality and inequality constraints
as special factors in the graph.  We validate our approach by
designing an \gls{mpc} controller that can be used as an elegant and
compact local planner.  In addition, we address the problem
of obstacle avoidance by designing a factor that relies on
a distance cost function inspired by scan registration techniques.
The modular nature of factor graphs allows us to jointly solve
 \gls{mpc} while addressing obstacle avoidance through our \gls{fgs}~\cite{grisetti2020solver}.
 

